Unifying Pointer Analyses for Polyglot Inter-operations through Summary Specialization

Modular analysis of polyglot applications is challenging because heap object flows across language boundaries must be resolved. The state-of-the-art analyses for polyglot applications have two fundamental limitations. First, they assume explicit boundaries between the host and the guest language to determine inter-language dataflows. Second, they rely on specific analyses of the host and guest languages. The former assumption is impractical concerning recent advancements in polyglot programming techniques, while the latter disregards advances in pointer analysis of the underlying languages. In this work, we propose to extend existing pointer analyses with a novel summary specialization technique so that points-to set across language boundaries can be unified. Our novel technique leverages various combinations of host and guest analyses with minor modifications. We demonstrate the efficacy and generalizability of our approach by evaluating it with two polyglot language models: Java-C communication via Android's NDK and Java-Python communication in GraalVM.

==> sections/info-flow.tex <==
In this section, we extend our modular analysis framework with a data flow analysis across language borders. Our extension assumes a security lattice, where each variable maps to a corresponding security label in the lattice. Our framework adopts the traditional security lattice, $\mathit{l} \sqsubseteq \mathit{h}$, where $\mathit{l}$ denotes public data while $\mathit{h}$ denotes confidential/sensitive data. Our language model assumes that sensitive sources and public sinks are present in both host and guest, i.e., the sensitive information can originate from the host and leak through the guest, and \textit{vice-versa}. A simple flow is demonstrated in~\Cref{fig:model}.   

\begin{figure}
\includegraphics[width=\columnwidth]{images/InformationFlowModel.pdf}
\caption{Model of Guest and Host languages}
\label{fig:model}
\end{figure}



The core part of our framework (Summary Specialization, Unification, and Summary injection) now works with point-to-sets where security labels are attached to the variables. Unification is similar to that described in summary unification (section~\ref{sec:summary-unification}) but incorporates an update to the security labels. It unifies the corresponding security labels by computing the meet of the labels. The remaining part of the analysis is analogous to the approach described earlier. \Cref{algo:inject-summary-ifcABC} demonstrates the upgraded version of \Cref{algo:inject-summary}, with the variables and heap objects being updated with the security labels obtained from the unification. Notably, the security label update is a strong update, i.e., the previous labels are discarded; Unification determines the appropriate security labels via the meet operation, allowing the summary injection to proceed with a strong update safely. 

\begin{algorithm}
    \caption{\textsc{InjectSummaryWithFlowLabel}}
    \label{algo:inject-summary-ifcABC}
    \KwIn{Projection $\mathcal{R}^f$,  pre-analysis $\mathcal{P}$ }
    \KwIn{Function Summary $\mathcal{F}^f$ of a function $f$ }
    \KwOut{updated  pre-Analysis $\mathcal{P}_{modular}$}
    $\mathit{changedVars} \leftarrow \emptyset$ \\
   Updated Projection $\mathcal{R}^f_\Delta\leftarrow \emptyset$ \\
    \ForAll{$(\mathit{accesspath}^{\textcolor{violet}{\ell'}}, \mathit{heap}) \in \mathcal{F}^f$}{ \label{algo:inject-summary-loop-beginAB}
        \If{$\mathit{accesspath}^{\textcolor{violet}{\ell'}}$ is a simple variable $\mathit{var}$}{
            $\mathcal{R}^f_\Delta = \mathcal{R}^f_\Delta \cup \{(\mathit{var}, \mathit{heap}, \mathit{ctxt})\}$  \label{algo:inject-summary-simple-varAB}  \\
        }
        \If{$\mathit{accesspath}^{\textcolor{violet}{\ell'}}$ is a field access x.f}{
            
                \Case{\textsc{FieldSensitive} analysis} {
                    $\mathcal{R}^f_\Delta = \mathcal{R}^f_\Delta \cup \{(o_i^{\textcolor{violet}{\ell'}},f,heap^{\textcolor{violet}{\ell'}}) \mid \forall o_i \in  \mathcal{P}(x)$\}  \label{algo:inject-summary-field-sensitiveAB} \\
                }
                \Case{\textsc{FieldBased} analysis}{
                    $\mathcal{R}^f_\Delta = \mathcal{R}^f_\Delta \cup \{(f,heap^{\textcolor{violet}{\ell'}})\}$ \label{algo:inject-summary-field-basedAB} \\
                }
                \Case{\textsc{FieldInsensitive} analysis}{
                    $\mathcal{R}^f_\Delta = \mathcal{R}^f_\Delta \cup \{(o_i^{\textcolor{violet}{\ell'}}, heap^{\textcolor{violet}{\ell'}}) \mid \forall o_i \in  \mathcal{P}(x)\}$ \label{algo:inject-summary-field-insensitiveAB} \\
                }
          
            
        }
        $\mathit{changedVars} \leftarrow \mathit{changedVars} \cup \{\mathit{accesspath}^{\textcolor{violet}{\ell'}}\}$ \\
    } \label{algo:inject-summary-loop-endA}
// Update the guest projection to include resolved host projection \\
     \ForEach{$f' \in G_{\mathit{guest}}$ invoking $f$, which is a bridge method} 
    {
    	// Propagate host function's ($f$) return variable to guest ($f'$), adapting variable name. \\
    	$	\mathcal{R}^{f'} = 	\mathcal{R}^{f'} \cup \mathcal{R}^f_\Delta[\$ \mathit{ret}]$ \\
    
	}
  $\mathcal{P}_{modular} = \mathcal{P} \cup \mathcal{R}^{f'}$
\end{algorithm}

\cref{fig:information-flow} shows the analysis of the example program with security labels. In this case, the access path $\texttt{i.secret}$ is updated to the label $h$, as $\texttt{i.secret}$ has label $h$ in \texttt{setSecret} and $l$ in \texttt{getSecret}. Summary unification updates the access path to the sensitive label $h$ denoted in red. Summary injection injects the unified summary into the pre-analysis and updates the security labels of the variables (compare~\cref{fig:analysis-visualization}). Therefore, the returning value of method \emph{getValue} obtains the correct security label. Based on the points-to-set resolution analysis, a taint analysis can query these points-to-sets~\cite {boomerang, Yannis2017-OOPSLA-PTaint, hybridprunning} for finding aliases and incorporate the information for taint-analysis. %


\begin{algorithm}
    \caption{\textsc{TaintAnalysisWithPointerQuery}}
    \label{algo:tainted-analysis-pointer}
    \KwIn{t: Tainted variable}
    \KwIn{$\mathcal{P}_{modular}$: Interlanguage analysis }
    \KwOut{$\mathit{taintedVars}$: Set of tainted variables}
    $\mathit{taintedVars} \leftarrow \{t\}$ \label{algo:tainted-analysis-pointer:1}\\
    $\mathit{WL} \rightarrow \{t\}$ \label{algo:tainted-analysis-pointer:2}\\
    \Repeat{$\mathit{WL} \neq \emptyset$}{ \label{algo:tainted-analysis-pointer:3}
        $t' \leftarrow \mathit{WL.pop()}$ \label{algo:tainted-analysis-pointer:4} \\ 
        $\mathit{mayAliases} \leftarrow \mathit{computeMayAlias}(\mathcal{P}_{modular}, t')$ \label{algo:tainted-analysis-pointer:5} \\
        $\mathit{taintedVars} \leftarrow \mathit{taintedVars}  \cup \mathit{mayAliases} $ \label{algo:tainted-analysis-pointer:6} \\
        $\mathit{WL} \leftarrow \mathit{WL} \cup \mathit{mayAliases}$ \label{algo:tainted-analysis-pointer:7} \\
    } \label{algo:tainted-analysis-pointer:8}
\end{algorithm}

\begin{figure}
    \centering
    \begin{adjustbox}{width=\columnwidth}
    	\centering
    \includegraphics[width=\textwidth]{images/InformationFlow.pdf}
\end{adjustbox}
    \caption{Unification with Information Flows}
    \label{fig:information-flow}
    \end{figure}

\Cref{algo:tainted-analysis-pointer} shows a naive approach for taint analysis with pointer queries. It recursively computes the may-aliases of the tainted variables. \Cref{algo:tainted-analysis-pointer:1} and \ref{algo:tainted-analysis-pointer:2} initialize the tainted variables and a worklist with the input taint variable $t$. ~\Cref{algo:tainted-analysis-pointer:3}-~\ref{algo:tainted-analysis-pointer:8} query the may-aliases information for input tainted variable $t$, and adds the results to the worklist. By computing the transitive closure of the tainted variable's may-aliases, the framework leverages the pointer analysis for taint analysis. In summary, the pointer analysis in our approach computes the flow labels of the variables participating in the inter-language communication, which enhances the precision of the pointer queries during taint analysis. 


